Data Poisoning Attacks and Defenses to Crowdsourcing Systems

A key challenge of big data analytics is how to collect a large volume of (labeled) data. Crowdsourcing aims to address this challenge via aggregating and estimating high-quality data (e.g., sentiment label for text) from pervasive clients/users. Existing studies on crowdsourcing focus on designing new methods to improve the aggregated data quality from unreliable/noisy clients. However, the security aspects of such crowdsourcing systems remain under-explored to date. We aim to bridge this gap in this work. Specifically, we show that crowdsourcing is vulnerable to data poisoning attacks, in which malicious clients provide carefully crafted data to corrupt the aggregated data. We formulate our proposed data poisoning attacks as an optimization problem that maximizes the error of the aggregated data. Our evaluation results on one synthetic and two real-world benchmark datasets demonstrate that the proposed attacks can substantially increase the estimation errors of the aggregated data. We also propose two defenses to reduce the impact of malicious clients. Our empirical results show that the proposed defenses can substantially reduce the estimation errors of the data poisoning attacks.

==> macros.tex <==

%
% The name of this file is ``macros.tex''
%

%
% TEX defaults
%
%
% frame 6.5 * 9
\textwidth 6.5in
\textheight 9in

% left/right margins
\oddsidemargin 0pt
\evensidemargin 0pt
\marginparwidth 1in
\marginparsep 0pt

% top margin
\topmargin -25pt
\headheight 10pt
\headsep 30pt
% \topskip 0pt

% foot margin
%\footheight 0pt
\footskip 27pt


% macros for commonly used special fonts
\newcommand{\IE}{{\it i.e.,}\ }
\newcommand{\EG}{{\it e.g.,}\ }
% single/double spacing
%\newcommand{\SS}{\renewcommand{\baselinestretch}{1}\large\normalsize}
\newcommand{\DS}{\renewcommand{\baselinestretch}{1.6}\large\normalsize}
% reduce the space between lines
\newcommand{\Tight}{\renewcommand{\baselinestretch}{0.9}\large\normalsize}
\newcommand{\HalfTight}{\renewcommand{\baselinestretch}{0.95}\large\normalsize}
\newcommand{\MinorTight}{\renewcommand{\baselinestretch}{0.975}\large\normalsize}
% Page title (primarily for foils)
% (this was called \HH}
\newcommand{\PageTitle}[1]{{\newpage \begin{center}{\LARGE {\bf {#1}} } \end{center} } }

% remove spaces around section headers
%\newcommand{\Section}[1]{\vspace{-3ex}\section{#1}\vspace{-2ex}}
\newcommand{\Subsection}[1]{\vspace{-2ex}\subsection{#1}\vspace{-1ex}}
\newcommand{\Subsubsection}[1]{\vspace{-2ex}\subsubsection{#1}\vspace{-1ex}}

% go forward n lines (negative for backward move)
\newcommand{\VLine}[1]{\vspace{#1ex}}
% itemize and enumerate without spaces around/between items
\newenvironment{TightItem}{\vspace{-2ex}\begin{itemize}
  \setlength{\itemsep}{-0ex}}{\end{itemize}\vspace{-1ex}}
\newenvironment{TightEnum}{\vspace{-2ex}\begin{enumerate}
  \setlength{\itemsep}{-0ex}}{\end{enumerate}\vspace{-1ex}}
\newenvironment{TightDesc}{\vspace{-1ex}\begin{description}
  \setlength{\itemsep}{-0ex}}{\end{description}\vspace{-1ex}}
% set the page number (to the first argument)
\newcommand{\SetPageNo}[1]{\countdef\pageno=0 \pageno=#1}
% things to do
\newenvironment{Todo}{\begin{large}\begin{bf}********** things to do
    ********** \\}{\\ **********\end{bf}\end{large}}
% for discussion
\newenvironment{Discuss}{\begin{large}\begin{em}**********
    things to be discussed ********** \\}{\\ **********\end{em}\end{large}}
% set the paragraph identation and separation


% the foil environment
\newenvironment{Foil}{\begin{document}\begin{LARGE}\begin{sf}
    }{\end{sf}\end{LARGE}\end{document}}
    % NOTE: ``}'' must be in the 2nd line
% foil page title
\newcommand{\Title}[1]{\newpage \center{\huge {\sf #1}} \flushleft
    \vspace{1ex}}

% set the paragraph identation and separation
\parindent 0.2in
\setlength{\parskip}{1ex}

% set text width
\textwidth = 6.75in

% set the formula separation
\setlength{\topsep}{0in}

% set indentation for formulas:
% \setlength{\mathindent}{3ex}

% set left margin
\setlength{\oddsidemargin}{-.1in}



